CoSINT: Designing a Collaborative Capture the Flag Competition to Investigate Misinformation

Crowdsourced investigations shore up democratic institutions by debunking misinformation and uncovering human rights abuses. However, current crowdsourcing approaches rely on simplistic collaborative or competitive models and lack technological support, limiting their collective impact. Prior research has shown that blending elements of competition and collaboration can lead to greater performance and creativity, but crowdsourced investigations pose unique analytical and ethical challenges. In this paper, we employed a four-month-long Research through Design process to design and evaluate a novel interaction style called collaborative capture the flag competitions (CoCTFs). We instantiated this interaction style through CoSINT, a platform that enables a trained crowd to work with professional investigators to identify and investigate social media misinformation. Our mixed-methods evaluation showed that CoSINT leverages the complementary strengths of competition and collaboration, allowing a crowd to quickly identify and debunk misinformation. We also highlight tensions between competition versus collaboration and discuss implications for the design of crowdsourced investigations.

==> 5_1-Findings-Background_and_Motives.tex <==


\subsection{Participants' Backgrounds, Motives, and Definitions of Success}
\label{sec:motives}

\subsubsection{Background and motives}

Many of the Computer Science students had prior exposure to cybersecurity courses and CTFs. DD-10, who had attended several cybersecurity CTFs, felt that using a CTF format ``is a really cool way to introduce people to the field'' of OSINT. KP-15 also described how OSINT was one of several categories in a cybersecurity CTF they attended and that ``those were the most fun ones, at least for me, to do.''

In contrast, none of the Political Science students had attended a CTF but had significant experience conducting OSINT investigations. For example, OT-1 said, ``I’ve been pretty active in OSINT. I feel like it’s one of the most accessible forms of intelligence that I think anyone can get into.''

We also found that students were drawn to the real-world nature of the class. For instance, DD-12 said he became interested in the class because he was ``looking for more opportunities to connect my computer science degree to real world applications \ldots and this just seemed like a good opportunity to do so in a very topical area.''

Several students also expressed an interest in learning more about OSINT investigations to combat misinformation. %

In addition, the Political Science students said that they were curious about the interdisciplinary nature of the class and wanted to develop more expertise in programming and with software tools.%





==> 5_4-Findings-Evidence_Flags.tex <==

\subsection{CoSINT Was Enjoyable to Use and Helped to Better Structure Investigations}

\subsubsection{Students enjoyed using CoSINT}
Many students, including SL-2, SS-4, KP-15, and KG-8, said they enjoyed using CoSINT. For example, KP-15 mentioned that one of his favorite things about using CoSINT is ``once you get into the flow state, it feels very intuitive. It’s very easy to get momentum going.'' He also valued the real-world impact CoSINT could have addressing the spread of misinformation compared to more theoretical CTFs, adding: ``I think it’s easier to see an impact and feel more fulfilled than just debugging system code \ldots you can feel there’s more of a sense of good and purpose.''


A few students, however, did not enjoy CoSINT as much. For instance, DD-11 wished that the CTFs were more focused on content quality rather than quantity, a point we return to in Section (XYZ): ``I personally haven’t gotten much out of the CTFs thus far just because you’re trying to throw as many things on the wall, and maybe something will stick. \ldots With how little time we were given, we weren’t able to find good pieces of [mis]information.''




\subsubsection{Improving CoSINT}
Students suggested areas where CoSINT's evidence and flag structure can be improved. We discuss other improvements related to judging, the point system, and the API, in their respective sections. 

In terms of structural changes, students wished that flags were organized in a way that they were easier to search, sort, filter, make sense of, and reuse. For instance, KG-8 said he felt confused by having four different flags for each evidence piece because this required him to read each flag to know what work was complete and what was remaining. While CoSINT supports multiple verification flags for the same evidence, enabling students to verify different part of a claim, SL-2 also wished that verification flags could be reused across different evidence pieces. This is because certain claims made by the same person or the same claim made by different people could all be verified or refuted by one reusable verification flag. 

KG-6 wanted flags to be organized differently because ``there's just so much information, it's [a lot of] scrolling'' towards the end of the CTF when a teams have submitted multiple flags. However, her teammates KG-8 and KG-9 admitted to not using the evidence view which might have made it easier to search through and make sense of. This suggests that the relationship between flags and evidence should be made clearer within CoSINT.

In terms of procedural changes, students suggested ways to make it easier to submit and process flags within CoSINT through additional tools and features. For example, DD-13 twice suggested a web browser extension to automatically capture information required to submit a discovery flag (e.g., creation date, number of likes or views, etc.) so that he could create a queue of discovery or verification flags that he could process in batches. SS-4, SL-2, DD-10, and KG-8 also wished for a feature to determine whether a piece of content had already been discovered and archived before because ``it ended up being a hunt and peck situation where I'd be like, 'vaccines are poison --- Control + F.' Is there an archive? Okay, there's not an archive, I'm good to make a flag'' (KG-8). This includes discoveries for the exact same URL, discoveries for the same content on different platforms, or discoveries for similar content.





==> 5_7-Findings-API.tex <==

\subsection{API Enabled Appropriation}
We designed CoSINT's API to allow participants to crowdsource tasks to other participants. Students created a variety of tools using CoSINT’s API supporting three of the four steps in the OSINT cycle (all but reporting). Most computer science students said that using the API was easy, however some pointed out that the API can be both freeing and constraining. %

\subsubsection{Types of tools enabled by the API}

\paragraph{Tools for discovery}
Students built TwitCat and CrowdSieve to support crowdsourced content discovery on Twitter and Reddit, respectively. TwitCat scraped tweets based on a user’s query and created tasks for crowd workers to label tweets for potential misinformation. TwitCat then aggregated, ranked, and displayed the crowd’s feedback to the user ``so that they might more quickly identify pieces of potential disinformation to explore further, alongside the [crowd workers’] rationale for their decision.'' KP-14, who used several teams’ tools during the final CTF, particularly admired TwitCat: ``I thought that was really cool. It inspired me, like that’s definitely something that we should have added to our platform to actually embed tweets.'' 

While TwitCat automatically scraped tweets, CrowdSieve relied upon crowd workers to search through subreddits manually. 
DD-13, whose team built CrowdSieve, said he would like to incorporate automation into the tool: ``Especially for things that might feel a little bit, maybe menial, or time consuming \ldots [have] investigators and intelligent software working in tandem.'' %

\paragraph{Tools for archiving}
KeyHive and HAL9001 were archival tools built by two different teams. KeyHive asked users to input an image URL and automatically archived it, then created tasks on CoSINT where crowd workers annotate each image. KeyHive then enables users to compare and search for images based on the crowd’s annotations. HAL9001 did not leverage crowdsourcing, but instead used automation (a Discord chat bot) to provide an alternative, natural language interface for querying CoSINT for tasks and flags. It also included a feature where users can enter a URL and automatically archive it. HAL9001 checks if the URL has already been submitted before, an additional feature that CoSINT does not offer.%


\paragraph{Tools for verification}
Of the four tools that teams built to support verification, two were focused on supporting verification on Twitter by using crowds to annotate popular hashtags and to annotate tweets from a given Twitter user. One tool, Photo Verification App, allowed a user to post an image that could be verified by other crowd workers. Credibility Checker included similar features but with a broader scope, supporting verifications of any type of content. SS-5, whose team built Credibility Checker, decided to focus on verification because ``that's the most time consuming step because you have to do a little bit more research'' thus allowing the ``investigator to focus on finding new flags or archiving previous discoveries while their volunteers determine the credibility of the flag sent to them.''

 
\subsubsection{Experiences using CoSINT's API}
For most students with a programming background, using the API was ``very straightforward'' (KP-14) --- perhaps because we provided code examples and documentation on how to use it. The political science students contributed domain expertise to user interface design and testing, but as DD-13 noted, some felt frustrated they could not contribute to writing code.

Three students also noted that CoSINT's API was simultaneously freeing and constraining. While most students used the API to build the expected crowdsourcing tools, we were surprised by the creativity of the HAL9001 team providing new types of UIs and augmenting CoSINT's capabilities. DD-12 noted how the API streamlined certain types of add-ons, but constrained imagination for others: ``I thought it was definitely cool how it handled the task management for you. \ldots But I definitely think more flexibility would be good because it would support more use cases, right?''



==> other.tex <==

@misc{noauthor_fake_nodate,
	title = {Fake {News} {Challenge}},
	url = {http://www.fakenewschallenge.org/},
	urldate = {2022-08-29}
}

@misc{noauthor_hunchly_nodate,
	title = {Hunchly - {OSINT} {Software} for {Cybersecurity}, {Law} {Enforcement}, {Journalists}, {Private} {Investigators} and more.},
	url = {https://www.hunch.ly/},
	urldate = {2022-08-29},
}

@misc{birdwatch, title={Twitter Birdwatch}, url={https://twitter.github.io/birdwatch/}, publisher={Twitter}
},

@inproceedings{venkatagiri2018response,
	title        = {Response to ``Heuristics for the Online Curator''},
	author       = {Venkatagiri, Sukrit and Zhang, Amy X},
	year         = 2018,
	journal      = {Curbing the Spread of Misinformation: Insights, Innovations, and Interpretations From the Misinformation Solutions Forum},
	publisher    = {RTI Press},
	address      = {Research Triangle Park, NC},
	pages        = {9--10},
	doi          = {https://doi.org/10.3768/rtipress.2018.cp.0008.1812},
	editor       = {Southwell, Brian G and Boudewyns, Vanessa}
}

@misc{gdilab2022uta,
	title = {The {Global} {Disinformation} {Lab} at the {University} of {Texas} at {Austin}},
	url = {https://gdil.org/},
	abstract = {The Global Disinformation Lab (GDIL) at the University of Texas at Austin. Disinformation and misinformation are global. So are we.},
	language = {en-US},
	urldate = {2022-08-29},
	journal = {GDIL {\textbar} Global Disinformation Lab at UT Austin},
	file = {Snapshot:/Users/sukritv/Zotero/storage/8K3G3MNM/gdil.org.html:text/html},
}
,

@misc{crowdtangle_crowdtangle_nodate,
	title = {{CrowdTangle} {\textbar} {Content} {Discovery} and {Social} {Monitoring} {Made} {Easy}},
	url = {https://www.crowdtangle.com//},
	abstract = {Request access to CrowdTangle!},
	language = {en},
	urldate = {2022-08-29},
	journal = {CrowdTangle},
	author = {CrowdTangle},
	file = {Snapshot:/Users/sukritv/Zotero/storage/4RW3ZGNN/www.crowdtangle.com.html:text/html},
}
